Power-Temperature Stability and Safety Analysis for Multiprocessor Systems

Modern multiprocessor system-on-chips (SoCs) integrate multiple heterogeneous cores to achieve high energy efficiency. The power consumption of each core contributes to an increase in the temperature across the chip floorplan. In turn, higher temperature increases the leakage power exponentially, and leads to a positive feedback with nonlinear dynamics. This paper presents a power-temperature stability and safety analysis technique for multiprocessor systems. This analysis reveals the conditions under which the power-temperature trajectory converges to a stable fixed point. We also present a simple formula to compute the stable fixed point and maximum thermally-safe power consumption at runtime. Hardware measurements on a state-of-the-art mobile processor show that our analytical formulation can predict the stable fixed point with an average error of 2.6%. Hence, our approach can be used at runtime to ensure thermally safe operation and guard against thermal threats.

==> files/fixed_point_prediction_backup.tex <==
\vspace{-1.5mm}
\section{Thermal Fixed Point Analysis} \label{sec:fixed_point_prediction}
%
Let the scalar $T$ denote the maximum steady state temperature 
over all thermal hotspots, i.e.:
\vspace{-1.5mm}
\begin{equation*}
T = \max_{1 \leq i \leq N} \lim_{k \rightarrow \infty} T_i[k] %~~
%\mathrm{where}~i~\mathrm{denotes~the}~i^{th}~\mathrm{hotspot}
\end{equation*}
%
\textcolor{red}{Since the thermal safety is determined maximum temperature, 
we focus on the hotspot with the largest temperature.}
At steady state ($k\rightarrow \infty$), we can model the temperature of \emph{each hotspot}
using the following single input single output (SISO) system: 
%
\topskip0pt 
\begin{equation}\label{eqn:temp_ss}
T = aT + bP
\end{equation}

\noindent where $0<a<1$ and $b>0$ are the parameters of the reduced order system. 
We emphasize that the reduced order model is obtained through system identification,
as described in Section~\ref{sec:sys_id}.
\textcolor{red}{Using a SISO model does not mean that we consider only one core. 
Unlike a crude approximation that directly uses the corresponding entries 
in $A$ and $B$ matrices, 
the coefficient $a$ in our model reflect the thermal coupling between different hotspots, 
and coefficient $b$ reflects the impact of multiple power sources. 
We employ a SISO model, since it enables in-depth theoretical analysis 
with powerful insights for practical scenarios.}
We discuss generalization to the multi input multi output (MIMO) case at the end of this section.

To isolate the impact of the temperature,
we re-write the total power consumption given in Equation~\ref{eqn:total_power} as:
%
\begin{equation}\label{eqn:power_simplifed}
P = P_C + V \kappa_{1}T^2e^{\frac{\kappa_{2}}{T}}
\end{equation}
%
where $P_C = C_{sw} V^2 f + V I_{g}$ represents the \emph{temperature independent} component,
and subscript $i$ is dropped to simplify the notation. 
Substituting Equation~\ref{eqn:power_simplifed} into Equation~\ref{eqn:temp_ss} gives:
%
\begin{equation} \label{fixed_point_ori}
(1-a)T - bP_C = bV \kappa_{1}T^2e^{\frac{\kappa_{2}}{T}}
\end{equation}
%
When this equation has feasible solution(s), 
then we can say that fixed points exist. 
Since Equation~\ref{fixed_point_ori} is the \textit{focal point} of the subsequent analysis, 
we introduce the following change of variables 
to leave the exponential term alone and facilitate the subsequent analysis:
%
\begin{equation} \label{change_of_parameters}
\hspace{-2mm} \T = -\frac{\kappa_2}{T}, \hspace{3mm} 
\alpha = \frac{b}{a-1}\frac{P_C}{\kappa_2} > 0, \hspace{3mm}
\beta =  \frac{a-1}{b} \frac{1}{V \kappa_{1} \kappa_{2}} > 0 \hspace{1mm}
\end{equation}
%
With this change of variables, we rewrite Equation~\ref{fixed_point_ori} as:
\begin{equation} \label{eqn:fixed_point}
\beta \T(1-\alpha\T)=e^{-\T}
\end{equation}
%
where $\alpha >0, \beta >0$.
\textit{\uline{We will first derive the conditions on $\alpha$ and $\beta$ such 
that
Equation~\ref{eqn:fixed_point} has a solution.}}
Then, we will go back from the transformed domain to the original parameters. 
Finally, we will show how to compute the constraint on the maximum power consumption $P_C^*$ 
required to avoid thermal violations, given a maximum temperature 
constraint $T^*$.


%\subsection{\hspace{-1mm}Domain of the Auxiliary Temperature $\T$}\label{aux_temp_domain}
%Physically feasible temperature $T$ (in $^\circ$K) $\in (0,\infty)$ and $\kappa_2 < 0$.
%The change of variables in Equation~\ref{change_of_parameters}
%implies $\T \in (0,\infty)$.
%Consequently, $e^{-\T}$, i.e., the right hand side of Equation~\ref{eqn:fixed_point}
%goes from is bounded within the interval $[0,1)$.
%Therefore, the following inequality holds:
%%0 \hspace{-0.25mm} < \hspace{-0.5mm} e^{-\T} \hspace{-1mm}<\hspace{-0.25mm} 1$.
%%Hence, Equation~\ref{eqn:fixed_point} has a solution, \textit{only if} the following %inequality holds:
%%
%\begin{equation*}
%0 < \beta \T(1-\alpha\T)< 1
%\end{equation*}
%%
%%Note that boundaries are not included since they correspond to $T=0$ and $T=\infty$ cases which are not physically feasible temperatures.
%The first inequality requires that $\T<1/\alpha$, whereas the second inequality implies the following quadratic inequality: % holds,
%%
%\[
%\beta \T(1-\alpha\T) < 1 \hspace{1mm} \Rightarrow  \hspace{2mm} 0 < (\T-0.5\alpha^{-1})^2-(0.25\alpha^{-1}-\beta^{-1})\alpha^{-1}
%\] Using these inequalities, we can find that Equation~\ref{eqn:fixed_point} has a feasible solution only for the following domain:
%%One can see that this equality is satisfied if
%\begin{equation} \label{eqn:domain}
%\left\{
%\begin{array}{ll}
%\T \in (0,1/ \alpha) ~&~ if~\beta<4\alpha \\
%\T \in (0,\frac{1}{2\alpha}-\Delta] \cup [\frac{1}{2\alpha}+\Delta,1 / \alpha) ~&~ if~\beta\geq4\alpha \\
%\end{array}
%\right.
%\end{equation}
%where $\Delta=\sqrt{(0.25\alpha^{-1}-\beta^{-1})\alpha^{-1}}$.
%
%%\noindent \textbf{Necessary and Sufficient Conditions for the Existence of Fixed Point: }
%%\setcounter{subsubsection}{1}

\subsection{Necessary and Sufficient Conditions for the Existence 
of Fixed Point(s)} \label{sec:fixed_point_condition}

The domain of the auxiliary temperature is given by $\T \in (0,\infty)$, 
since $\T = -\kappa_2 /T$ where $\kappa_2 < 0$. 
Hence, the right hand side of Equation~\ref{eqn:fixed_point} 
lies in the interval $(0,1)$. 
That is, $0 < \beta \T(1-\alpha\T) = e^{-\T} < 1$. 
Since this condition requires that $\T<1/\alpha$, 
we can take the logarithm of both sides while the equality holds, i.e.,
%\vspace{-2mm}
\[
\ln \beta + \ln \T + \ln(1-\alpha \T) = -\T
\]
Equation~\ref{eqn:fixed_point} has the same fixed points as the following equation: 
%
\begin{equation} \label{eqn:fixed_point_ln}
\mathcal{F}(\T) \triangleq \ln \beta + \ln \T + \ln(1-\alpha \T) + \T = 0
\end{equation}
%
The following lemma summarizes the important properties of $\mathcal{F}(\T)$ 
employed in our analysis.
%
\begin{lemma} \label{lemma_F_T}
$\mathcal{F}(\T)$ given in Equation~\ref{eqn:fixed_point_ln} satisfies the following properties:
%
\begin{enumerate} [leftmargin=*]
  \item $\mathcal{F}(\T)$ is a concave function in the interval $\T \in 
  (0,1/\alpha)$,
  \item $\mathcal{F}(\T)$ has a unique maxima at $\T_m$, which is given by
%
\begin{equation} \label{eqn:inflection_point}
\T_m = \frac{1}{2\alpha}-1+\sqrt{\frac{1}{4\alpha^2}+1}
\end{equation}
% 
  \item $\mathcal{F}(\T)$ is an increasing function in the interval $(0,\T_m)$ and 
    a decreasing function in $(\T_m,1/\alpha)$
\end{enumerate}
%
\end{lemma}
%
\vspace{-5mm}
\textcolor{red}{
\begin{proof}
	The proof is provided in Appendix~\ref{proof_F_T}, 
	while an informal explanation is provided below to maintain a smooth flow.
\end{proof}
}
\vspace{-1mm}

Figure~\ref{fixed_point_illustration} sketches $\mathcal{F}(\T)$ for $\T \in (0, 1/ \alpha)$.
As the first two properties of Lemma~\ref{lemma_F_T} state, 
$\mathcal{F}(\T)$ is concave and has a unique maxima. 
Furthermore, it is increasing in the interval $(0,\T_m)$ and decreasing in 
$(\T_m,1/\alpha)$. 
As shown in Figure~\ref{fixed_point_illustration}, 
$\mathcal{F}(\T)$ reaches its peak at $\T=\T_m$. 
Hence, Equation~\ref{eqn:fixed_point_ln} ($\mathcal{F}(\T) = 0$)  
has \emph{two solutions} if and only if the maxima is non negative, i.e., 
$\mathcal{F}(\T_m) \geq 0$. 
%(case 1 in Figure~\ref{fixed_point_illustration}). 
The fixed points coincide when $\mathcal{F}(\T_m) = 0$, 
and there are no fixed points for $\mathcal{F}(\T_m) < 0$. 
To be practical, these conditions should be expressed 
in terms of the design parameters $\alpha$ and $\beta$.  
This is achieved by Theorem~\ref{thm_fixed_point}, which summarizes our first major result.

%
\begin{figure}[b]
	\vspace{-3mm}
	\centering
	\includegraphics[width=0.99\linewidth]{figures/illustration_new.pdf}
	\vspace{-5mm}
	\caption{Illustration of $\mathcal{F}(\T)$ when there is no fixed point and when there are two fixed points respectively.}
	\label{fixed_point_illustration}
	\vspace{-3mm}
\end{figure}
%
 
\begin{theorem} \label{thm_fixed_point} 
The maxima of $\mathcal{F}(\T)$ is given by:
\vspace{-1mm}
\begin{equation} \label{eqn:F_Tm}
\mathcal{F}(\T_m) = \ln \beta - \ln\left(\frac{2}{\T_m}+1 \right)e^{-\T_m}
\end{equation}
%
Hence, Equation~\ref{eqn:fixed_point} has two fixed points if and only if $\beta\geq\left(\frac{2}{\T_m}+1\right)e^{-\T_m}$ where $\T_m$
depends only the parameter $\alpha$ and defined in Equation~\ref{eqn:inflection_point}.
Otherwise, it has no solution.
\end{theorem}
%
\vspace{-3mm}
\begin{proof}
The proof is provided in Appendix~\ref{existence_proof}.
\end{proof}
\vspace{-3mm}

At runtime, we first compute $\T_m$ using Equation~\ref{eqn:inflection_point}. 
Then, we check the condition given in Theorem~\ref{thm_fixed_point}. 
If it is not satisfied, we conclude that there will be a thermal runaway. 
This knowledge can be used to throttle the cores aggressively or enter an 
emergency state. 
Otherwise, we proceed to compute the maximum allowed power consumption 
that will avoid thermal violations. 


\input{files/fixed_point_Suat.tex}

\subsection{Time to Reach the Stable Fixed Point}\label{sec:time_to_fp}
Once we determine the existence of a stable fixed point, 
we can also estimate the time it will take to reach the stable fixed point.
This estimate can aid DTPM policies 
to decide how long the current power consumption can be sustained 
without violating the thermal limit. 
To obtain a computationally efficient estimation, we employ the following exponential model:
%
\begin{equation}\label{eqn:exponential_model}
T[kT_s] = T_{init} + (T_{fix} - T_{init})(1 - e^{-\frac{kT_s}{\tau}})
\end{equation}
%
where $T_{init}$ is the initial temperature, $T_{fix}$ is the stable fixed 
point and $\tau$ is the time constant. 
We use the discrete time stamp $kT_s$, since the temperature is sampled with a 
period of $T_s$. 
Two temperature readings 
separated by a delay, i.e., $T[kT_s]$ and $T[(k-D)T_s]$,
can be used to estimate the time constant $\tau$ as:
%
\begin{equation}\label{eqn:tau_model}
\tau = \frac{t[kT_s] - t[(k-D)T_s]}{\ln(\frac{T[(k-D)T_s] - T_{fix}}{T[kT_s] - T_{fix}})}
\end{equation}
%
In our experiments, we set $T_s =100$~ms and $D=10$, i.e., 
the time constant estimate is updated once every second. 
Finally, we use $5\tau$ to reach within $1\%$ of the fixed point. 
Tighter or looser bounds can be used depending on the application scenario. 












































==> files/mimo_extension.tex <==
\subsection{\hspace{-3mm}Generalization to MIMO Case} \label{sec:mimo}
The SISO model given in Equation~\ref{eqn:temp_ss} can be extended 
to account for the impact of each power source on the thermal hotspot 
of interest $T_i$, as follows:
%
\begin{eqnarray*} \label{eqn:temp_miso}
T_i &=& aT_i + [b_1, b_2, \ldots, b_M] \mathbf{P[k]} \\
&=& aT_i + [b_1, b_2, \ldots, b_M] [P_1, P_2, \ldots, P_M]^\intercal \nonumber
\end{eqnarray*}
where $P_i$ terms are defined in Equation~\ref{eqn:total_power}.
%
The fixed point temperatures computation requires the solution of the set of equations,
\begin{eqnarray}
\mathbf{f(\bar T)}=\mathbf{f}(T_1,\ldots,T_M)=\left[\begin{array}{c}
f_1(T_1,\ldots,T_M) \\
\vdots \\
f_M(T_1,\ldots,T_M) 
\end{array}\right]=0
\end{eqnarray} where for $1\leq i \leq M$,
\[
f_i(T_1,\ldots,T_M)=(a-1)T_i + [b_1, b_2, \ldots, b_M] [P_1, P_2, \ldots, P_M]^\intercal
\]
This is a nonlinear equation due to the exponential terms in $P_i$. %terms 
We solve this equation via Newton's method with a good initial point for temperatures, 
as we outline in Algorithm~\ref{alg:mimo} below
%(for Newton's method, see Algorithm $9.5$ at page $487$ in \cite{boydoptbook}). 
~\cite{boydoptbook}.
% 
\begin{algorithm} Compute the fixed point temperatures for power decoupled 
	case, i.e., the initial points $\bar T_0$ and set $k\leftarrow 0$. \\
	\textbf{repeat} \label{alg:mimo}
	\begin{enumerate}[leftmargin=*]
		\item Compute the Newton step and decrement. \\
		$\Delta \bar T :=-\nabla^2f(\bar T_k)^{-1} \nabla f(\bar T_k)$; \\
		(where $\nabla f(\bar T)$ is the gradient and $\nabla^2 f(\bar T)$ is 
		the Hessian matrix) \\
		$\lambda^2:=\nabla f(\bar T_k)^T \nabla^2 f(\bar T_k)^{-1} \nabla 
		f(\bar T_k)$.   
		\item Stopping criterion. quit if $\lambda^2/2\leq\textrm{tolerance}$.
		\item Line search. Choose step size t by backtracking line search.
		\item Update. $\bar T_{k+1} := \bar T_{k} + t\Delta \bar T$, $k\leftarrow k+1$.
	\end{enumerate}
	$\bar T_k$ is the fixed point temperatures for power coupled case.
\end{algorithm}

As the experimental results demonstrate, the SISO results provide very good match with hardware measurements. 
Therefore, we  use our solution for the SISO case to compute the fixed point temperature for each thermal hotspot separately.  
Then, we use these temperatures as initial points to computed the fixed point temperatures for MIMO system, 
as outlined in Algorithm~\ref{alg:mimo}.
In addition to this, 
we are interested in the stability properties of fixed point temperatures and their convergence intervals. 
This is left for future work since it deserves a comprehensive study on its own.
%

%The notations $\nabla f(\bar T)$ and $\nabla f^2(\bar T)$ are the gradient and 
%Hessian of the function $f(\bar T)$ (see pages $69$-$71$ in \cite{boydoptbook} 
%for definitions and discussion).

 
